Stuttering Conway Sequences Are Still Conway Sequences

A look-and-say sequence is obtained iteratively by reading off the digits of the current value, grouping identical digits together: starting with 1, the sequence reads: 1, 11, 21, 1211, 111221, 312211, etc. (OEIS A005150). Starting with any digit $d \neq 1$ gives Conway's sequence: $d$, $1d$, $111d$, $311d$, $13211d$, etc. (OEIS A006715). Conway popularised these sequences and studied some of their properties. In this paper we consider a variant subbed "look-and-say again" where digits are repeated twice. We prove that the look-and-say again sequence contains only the digits $1, 2, 4, 6, d$, where $d$ represents the starting digit. Such sequences decompose and the ratio of successive lengths converges to Conway's constant. In fact, these properties result from a commuting diagram between look-and-say again sequences and "classical" look-and-say sequences. Similar results apply to the "look-and-say three times" sequence.

==> img/forest.tex <==
\begin{tikzpicture}
\node (1) at (0, 0) {\phantom{\dig{00}}\dig{1}};
\node (11) at (1.5, 0) {\dig{11}};
\node (21) at (3, 0) {\dig{21}};
\node (111) at (0, -1) {\dig{111}};
\node (31) at (3, -1) {\dig{31}};
\node (222) at (0, -2) {\dig{222}};
\node (0) at (0, -3) {\phantom{\dig{00}}\dig{0}};
\node (10) at (3, -3) {\dig{10}};
\node (00) at (5, -3) {\dig{00}};
\node (20) at (8, -3) {\phantom{\dig{0}}\dig{20}};
\node (000) at (2.5, -4) {\dig{000}};
\node (30) at (5.5, -4) {\dig{30}};
\node (32) at (3, -2) {\dig{32}};
\node (2) at (5, 0) {\phantom{\dig{0}}\dig{2}};
\node (22) at (7, 0) {\dig{22}};
\node (3) at (5, -2) {\phantom{\dig{0}}\dig{3}};
\node (33) at (6.5, -2) {\dig{33}};
\node (333) at (8, -2) {\dig{333}};
\draw[>=latex,->] (0) to node[above,midway,scale=0.8]{$Z$} (10);
\draw[>=latex,->] (00) to node[above,midway,scale=0.8]{$Z$} (20);
\draw[>=latex,->] (000) to node[above,midway,scale=0.8]{$Z$} (30);
\draw[>=latex,->] (1) to node[above,midway,scale=0.8]{$Z$} (11);
\draw[>=latex,->] (11) to node[above,midway,scale=0.8]{$Z$} (21);
\draw[>=latex,->] (111) to node[above,midway,scale=0.8]{$Z$} (31);
\draw[>=latex,->] (222) to node[above,midway,scale=0.8]{$Z$} (32);
\draw[>=latex,->] (2) to node[above,midway,scale=0.8]{$Z$} (22);
\draw[] (22) to[in=90,out=25] node[pos=1,right,scale=0.8]{$Z$} (8.5, 0);
\draw[>=latex,->] (8.5, 0) to[out=-90,in=-25] (22);
\draw[>=latex,->] (3) to node[above,midway,scale=0.8]{$Z$} (33);
\draw[>=latex,->] (333) to node[above,midway,scale=0.8]{$Z$} (33);
\draw[] (33) to[out=120,in=-180] node[pos=2,right,midway,scale=0.8]{$~Z$} (6.5, -1);
\draw[>=latex,->] (6.5, -1) to[out=0,in=60] (33);
\end{tikzpicture}
